An Unconditionally Energy-Stable Scheme Based on an Implicit Auxiliary Energy Variable for Incompressible Two-Phase Flows with Different Densities Involving Only Precomputable Coefficient Matrices

We present an energy-stable scheme for numerically approximating the governing equations for incompressible two-phase flows with different densities and dynamic viscosities for the two fluids. The proposed scheme employs a scalar-valued auxiliary energy variable in its formulation, and it satisfies a discrete energy stability property. More importantly, the scheme is computationally efficient. Within each time step, it computes two copies of the flow variables (velocity, pressure, phase field function) by solving individually a linear algebraic system involving a constant and time-independent coefficient matrix for each of these field variables. The coefficient matrices involved in these linear systems only need to be computed once and can be pre-computed. Additionally, within each time step the scheme requires the solution of a nonlinear algebraic equation about a {\em scalar-valued number} using the Newton's method. The cost for this nonlinear solver is very low, accounting for only a few percent of the total computation time per time step, because this nonlinear equation is about a scalar number, not a field function. Extensive numerical experiments have been presented for several two-phase flow problems involving large density ratios and large viscosity ratios. Comparisons with theory show that the proposed method produces physically accurate results. Simulations with large time step sizes demonstrate the stability of computations and verify the robustness of the proposed method. An implication of this work is that energy-stable schemes for two-phase problems can also become computationally efficient and competitive, eliminating the need for expensive re-computations of coefficient matrices, even at large density ratios and viscosity ratios.

==> AppendE.tex <==

\section*{Appendix E. Algorithm for N-Phase Momentum Equations}

We summarize the algorithm developed in \cite{Dong2015}
for the N-phase momentum equations,
which is employed in the current work.
The algorithm is for the equations \eqref{equ:nse_trans_1}
and \eqref{equ:continuity_original}, together
with the boundary condition \eqref{equ:bc_vel}.
It is assumed that the volume fractions $c_i^{n+1}$ ($1\leqslant i\leqslant N$)
and the auxiliary variables $\psi_i^{n+1}$ ($1\leqslant i\leqslant N$)
have already been computed using the algorithm presented
in Section \ref{sec:alg}.
The goal here is to compute the velocity $\mathbf{u}^{n+1}$ 
and the pressure $P^{n+1}$
with given $\mathbf{u}^n$, $P^n$, $c_i^{n+1}$ and $\psi_i^{n+1}$.


The algorithm consists of two steps. The pressure and the velocity
are computed successively in a de-coupled fashion in the first and the second
steps, respectively. \\
\noindent\underline{For $P^{n+1}$:}
\begin{subequations}
\begin{equation}
\begin{split}
\frac{\gamma_0\tilde{\mathbf{u}}^{n+1}-\hat{\mathbf{u}}}{\Delta t}
+ \mathbf{u}^{*,n+1}\cdot\nabla\mathbf{u}^{*,n+1}
& + \frac{1}{\rho^{n+1}}\tilde{\mathbf{J}}^{n+1}\cdot\nabla\mathbf{u}^{*,n+1}
+ \frac{1}{\rho_0}\nabla P^{n+1}
= 
\left(\frac{1}{\rho_0}-\frac{1}{\rho^{n+1}}  \right)\nabla P^{*,n+1} \\
& - \frac{\mu^{n+1}}{\rho^{n+1}}\nabla\times\nabla\times\mathbf{u}^{*,n+1}
+ \frac{1}{\rho^{n+1}}\nabla\mu^{n+1}\cdot\mathbf{D}(\mathbf{u}^{*,n+1}) \\
& - \frac{1}{\rho^{n+1}}\sum_{i,j=1}^{N}\lambda_{ij}\left(\psi_j^{n+1}-\alpha c_j^{n+1}\right)\nabla c_i^{n+1}
+ \frac{1}{\rho^{n+1}}\mathbf{f}^{n+1},
\end{split}
\label{equ:pressure_1}
\end{equation}
%
\begin{equation}
\nabla\cdot\tilde{\mathbf{u}}^{n+1} = 0,
\label{equ:pressure_2}
\end{equation}
%
\begin{equation}
\left.\mathbf{n}\cdot\tilde{\mathbf{u}}^{n+1}\right|_{\partial\Omega}
= \mathbf{n}\cdot\mathbf{w}^{n+1}.
\label{equ:pressure_3}
\end{equation}
\end{subequations}
%
\\
\noindent\underline{For $\mathbf{u}^{n+1}$:}
\begin{subequations}
\begin{equation}
\frac{\gamma_0\mathbf{u}^{n+1}-\gamma_0\tilde{\mathbf{u}}^{n+1}}{\Delta t}
 - \nu_0 \nabla^2\mathbf{u}^{n+1}
= \nu_0 \nabla\times\nabla\times\mathbf{u}^{*,n+1},
\label{equ:velocity_1}
\end{equation}
%
\begin{equation}
\left.\mathbf{u}^{n+1}  \right|_{\partial\Omega} = \mathbf{w}^{n+1}.
\label{equ:velocity_2}
\end{equation}
\end{subequations}


In the above equations all the symbols follow
the same notation as outlined in Section \ref{sec:alg}.
$\mathbf{u}^{*,n+1}$ and $P^{*,n+1}$
are defined by \eqref{equ:def_var_star}.
$\hat{\mathbf{u}}$ and $\gamma_0$ are defined
by \eqref{equ:def_var_hat}.
$\tilde{\mathbf{J}}^{n+1}$ is
given by (see equation \eqref{equ:H_expr})
\begin{equation}
\tilde{\mathbf{J}}^{n+1} = -\sum_{i,j=1}^N \tilde{\rho}_i m_{ij}(\vec{c}^{n+1})
\nabla\left[
  -\sum_{k=1}^N\lambda_{jk}(\psi_k^{n+1}-\alpha c_k^{n+1})
  + \mathscr{H}_j(\vec{c}^{n+1})
\right].
\label{equ:J_expr_1}
\end{equation}
Note that in both the above equation and in equation
\eqref{equ:pressure_1} we have replaced
$\nabla^2c_i^{n+1}$ by
($\psi_i^{n+1}-\alpha c_i^{n+1}$) according to equations 
\eqref{equ:CH_phi} and \eqref{equ:def_psi_N}. 
%
$\mathbf{n}$ is the outward-pointing unit vector
normal to $\partial\Omega$.
$\tilde{\mathbf{u}}^{n+1}$ is an auxiliary
velocity that approximates $\mathbf{u}^{n+1}$.
$\rho^{n+1}$ and $\mu^{n+1}$ are
given by \eqref{equ:rho_expr} and \eqref{equ:mu_expr},
and in case of large density ratios we follow \cite{Dong2015}
and further clamp
the values of $\rho^{n+1}$ and $\mu^{n+1}$ as follows
(see \cite{Dong2015} for details)
\begin{equation}
    \rho^{n+1} = \left\{
    \begin{array}{ll}
      \rho^{n+1}, & \text{if} \ \rho^{n+1}\in[\tilde{\rho}_{\min},\tilde{\rho}_{\max}] \\
      \tilde{\rho}_{\max}, & \text{if} \ \rho^{n+1} > \tilde{\rho}_{\max} \\
      \tilde{\rho}_{\min}, & \text{if} \ \rho^{n+1} < \tilde{\rho}_{\min},
    \end{array}
    \right.
    \quad
    \mu^{n+1} = \left\{
    \begin{array}{ll}
      \mu^{n+1}, & \text{if} \ \mu^{n+1}\in[\tilde{\mu}_{\min},\tilde{\mu}_{\max}] \\
      \tilde{\mu}_{\max}, & \text{if} \ \mu^{n+1} > \tilde{\mu}_{\max} \\
      \tilde{\mu}_{\min}, & \text{if} \ \mu^{n+1} < \tilde{\mu}_{\min},
    \end{array}
    \right.
    \label{equ:rho_mu_clamp}
  \end{equation}
  where
  $\tilde{\rho}_{\max} = \max_{1\leqslant i\leqslant N}\{\tilde{\rho}_i\}$,
  $\tilde{\rho}_{\min} = \min_{1\leqslant i\leqslant N}\{\tilde{\rho}_i\}$,
  $\tilde{\mu}_{\max} = \max_{1\leqslant i\leqslant N}\{\tilde{\mu}_i\}$,
  and $\tilde{\mu}_{\min} = \min_{1\leqslant i\leqslant N}\{\tilde{\mu}_i\}$.
%
The constant $\rho_0$ is given by
$ %\begin{equation}
\rho_0 = \tilde{\rho}_{\min} = \min_{1\leqslant i\leqslant N}\{\tilde{\rho}_i\}.
%\label{equ:rho_0_condition}
$ %\end{equation}
$\nu_0$ in \eqref{equ:velocity_1} is a chosen positive
constant that is sufficiently large.
We  employ an $\nu_0$ value
with the following property,
$ %\begin{equation}
\nu_0 \geqslant \max\left(
\frac{\tilde{\mu}_1}{\tilde{\rho}_1},
\frac{\tilde{\mu}_2}{\tilde{\rho}_2},
\cdots,
\frac{\tilde{\mu}_N}{\tilde{\rho}_N}
\right).
%\label{equ:nu_0_condition}
$ %\end{equation}


The above algorithm employs a velocity
correction-type idea \cite{DongS2010,DongKC2014,Dong2015clesobc}  to de-couple
the computations for the pressure and the velocity.
%It can be noted that the variable density $\rho$
%and the variable dynamic viscosity $\mu$ have been
%treated with a reformulation of
%the pressure term $\frac{1}{\rho}\nabla P$
%and a reformulation of the 
%viscous term $\frac{\mu}{\rho}\nabla^2\mathbf{u}$,
%so that 
With this algorithm the linear
algebraic systems resulting from the discretization
involve only {\em constant} and {\em time-independent} 
coefficient matrices, like
in two-phase flows \cite{DongS2012,Dong2012,Dong2014obc}. 
%The ideas for the reformulations stem from the original developments for
%two-phase flows \cite{DongS2012,Dong2012,Dong2014obc}.

It is straightforward to derive
the weak forms for the pressure and the velocity
for the implementation of the algorithm using
$C^0$ spectral elements; see \cite{Dong2015} for details. 
We only provide the final weak forms here.
% 
Let $q\in H^1(\Omega)$ denote the test function, and 
\begin{multline}
\mathbf{G}^{n+1} = 
\frac{1}{\rho^{n+1}}\mathbf{f}^{n+1}
- \left(
     \mathbf{u}^{*,n+1} 
     + \frac{1}{\rho^{n+1}} \tilde{\mathbf{J}}^{n+1}
  \right)\cdot\nabla\mathbf{u}^{*,n+1}
+ \frac{\hat{\mathbf{u}}}{\Delta t}
+ \left(\frac{1}{\rho_0} - \frac{1}{\rho^{n+1}}  \right)\nabla P^{*,n+1} \\
+ \frac{1}{\rho^{n+1}}\nabla\mu^{n+1}\cdot\mathbf{D}(\mathbf{u}^{*,n+1})
- \frac{1}{\rho^{n+1}}\sum_{i,j=1}^{N}\lambda_{ij}(\psi_j^{n+1}-\alpha c_j^{n+1})\nabla c_i^{n+1}
+ \nabla\left( \frac{\mu^{n+1}}{\rho^{n+1}} \right) \times \bm{\omega}^{*,n+1},
\label{equ:G_expr}
\end{multline}
where $\bm{\omega} = \nabla\times \mathbf{u}$ is
the vorticity.
The weak form for the pressure $P^{n+1}$ is
\begin{equation}
\int_{\Omega} \nabla P^{n+1} \cdot\nabla q
= \rho_0 \int_{\Omega} \mathbf{G}^{n+1}\cdot\nabla q
- \rho_0 \int_{\partial\Omega} \frac{\mu^{n+1}}{\rho^{n+1}} \mathbf{n}\times\bm{\omega}^{*,n+1}\cdot\nabla q
- \frac{\gamma_0\rho_0}{\Delta t}\int_{\partial\Omega}\mathbf{n}\cdot\mathbf{w}^{n+1} q,
\ \
\forall q\in H^1(\Omega).
\label{equ:p_weakform}
\end{equation}
%
Let 
$
H^1_0(\Omega) = \left\{ \
v \in H^1(\Omega) \ : \
v|_{\partial\Omega} = 0
\ \right\},
$
and $\varphi \in H_0^1(\Omega)$ denote
the test function.
The weak form about the velocity $\mathbf{u}^{n+1}$ is
\begin{multline}
\int_{\Omega}\nabla\varphi\cdot\nabla\mathbf{u}^{n+1}
+ \frac{\gamma_0}{\nu_0\Delta t}\int_{\Omega}\varphi\mathbf{u}^{n+1}
= \frac{1}{\nu_0}\int_{\Omega}\left(
    \mathbf{G}^{n+1} - \frac{1}{\rho_0}\nabla P^{n+1}
  \right) \varphi \\
- \frac{1}{\nu_0}\int_{\Omega} \left(
    \frac{\mu^{n+1}}{\rho^{n+1}} - \nu_0
  \right) 
  \bm{\omega}^{*,n+1} \times \nabla\varphi,
\qquad
\forall \varphi \in H_0^1(\Omega).
\label{equ:vel_weakform}
\end{multline}
%
These weak forms, 
\eqref{equ:p_weakform} and
\eqref{equ:vel_weakform}, can be
discretized in space using $C^0$ spectral 
elements 
in a straightforward
fashion~\cite{Dong2015}. 


Solving the N-phase momentum equations
\eqref{equ:nse_trans_1} and \eqref{equ:continuity_original}
amounts to the following two successive operations. First,
solve equation \eqref{equ:p_weakform} for
pressure $P^{n+1}$. Then, solve
equation \eqref{equ:vel_weakform}, together with
the Dirichlet condition \eqref{equ:velocity_2} on $\partial\Omega$,
for $\mathbf{u}^{n+1}$.







